ProvNeRF: Modeling per Point Provenance in NeRFs as a Stochastic Field

Neural radiance fields (NeRFs) have gained popularity with multiple works showing promising results across various applications. However, to the best of our knowledge, existing works do not explicitly model the distribution of training camera poses, or consequently the triangulation quality, a key factor affecting reconstruction quality dating back to classical vision literature. We close this gap with ProvNeRF, an approach that models the \textbf{provenance} for each point -- i.e., the locations where it is likely visible -- of NeRFs as a stochastic field. We achieve this by extending implicit maximum likelihood estimation (IMLE) to functional space with an optimizable objective. We show that modeling per-point provenance during the NeRF optimization enriches the model with information on triangulation leading to improvements in novel view synthesis and uncertainty estimation under the challenging sparse, unconstrained view setting against competitive baselines.

==> sections/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Neural radiance fields (NeRFs)~\cite{mildenhall2020nerf} have increasingly grown in popularity in the recent years, touching different applications in novel view synthesis~\cite{barron2021mipnerf, barron2023zipnerf}, depth estimation~\cite{deng2022depthsupervised}, robotics~\cite{IchnowskiAvigal2021DexNeRF, nerf-nav}, localization~\cite{liu2023nerfloc, maggio2022locnerf}, etc. However, NeRFs struggle in the sparse-view regime due to inadequate constraints from volume rendering alone~\cite{Niemeyer2021Regnerf, sparf2023, wang2023sparsenerf}. Despite the challenges, such views are easier in practice to obtain by user-friendly methods, such as when capturing images in-the-wild with a smartphone. Therefore, understanding a 3D scene given \emph{sparse}~\cite{8637125}, \emph{unconstrained}~\cite{10.1145/1141911.1141964} camera views is an important problem dating back to classical computer vision with multiple applications such as in structure-from-motion~\cite{5459148, 9879641}, SLAM~\cite{Matsuki2021CodeMappingRD, 7898369} and uncertainty estimation~\cite{uncmodel00, 9879715}. 


% Original neural radiance fields rely on a dense set of views to achieve photorealistic 3D reconstruction. Under an under-constraint setting such as a sparse, unconstrained set of inputs, NeRFs' optimization is prone to local minima and frequently results 

Original neural radiance fields rely solely on photometric consistency across different views to recover geometry and appearance. Thus, photorealistic 3D reconstruction requires careful selection of input views so that every part of the scene is well-triangulated. Under a sparse setting, this is even harder to achieve because of the limited number of training cameras. As a result, regions with poor triangulation will result in unrealistic novel view synthesis (NVS) and 3D reconstruction. Existing works have tackled this issue from two angles. One line of work introduces additional priors to the sparse view NeRF optimization such as depth~\cite{deng2022depthsupervised, scade, roessle2022depthpriorsnerf}, structure similarities~\cite{Niemeyer2021Regnerf, Yang2023FreeNeRF, Jain_2021_ICCV}, and global shape information~\cite{jang2021codenerf, rematasICML21, Yuan2023InteractiveNG}. These works, however, do not explicitly account for the training camera poses during optimization despite triangulation being one of the major factors affecting NVS quality. The other line of work estimates NeRF's uncertainty to pinpoint the region of poor reconstruction~\cite{bayesrays, pan2022activenerf, jiang2023fisherrf, sünderhauf2022densityaware, CF-NeRF, s-nerf}. Yet again, none of these works specifically measures the uncertainty caused by training camera triangulation despite its importance in NeRF's optimization. 

% a more efficient quantification that can be especially useful for tasks such as next-view augmentation. \george{should I say this here?} \mika{Can we back the usefulness of uncertainty in the capture process? If it's not that strong, maybe this can go into RW instead of intro -- at least not a full paragraph in the intro.}
% \mika{I like this ``however, do not explicitly take training camera displacements and poses into account during optimization despite their critical role in the NeRF's optimization". We might be able to upsell this if experiments back it. It should go into the abstract. We probably just don't want to say its ``understanding a 3D scene" (at least not too much) as that seems confusing.}

% are designed specifically to improve novel view synthesis and ignore the inherent reconstructio ambiguity caused by the displacements of training camera poses~\cite{hartley_zisserman_2004}. 

% In a different line of work, the uncertainty of underconstrained NeRFs is studied and quantified using Bayesian analysis~\cite{bayesrays, pan2022activenerf, jiang2023fisherrf}, ensemble learning~\cite{sünderhauf2022densityaware}, and variational inference~\cite{CF-NeRF, s-nerf}. Yet again, none of these works specifically measures the uncertainty caused by training camera triangulation, but instead entangle different sources of uncertainty from triangulation, model convergence, and data inconsistencies together. While such an entangled quantification can be useful in many situations, a triangulation-specific uncertainty would lead to a more efficient quantification that can be especially useful for tasks such as next-view augmentation. \george{should I say this here?} \mika{Can we back the usefulness of uncertainty in the capture process? If it's not that strong, maybe this can go into RW instead of intro -- at least not a full paragraph in the intro.}
% \mika{Need to word this better:}
%However, there are other important problems that arise under this setting such as uncertainty estimation, viewpoint selection and the like.
% In this work we show that multiple such questions under the sparse, unconstrained view regime can be addressed by asking the question: ``from where has each point been seen?", and this information can be obtained for free from the training camera poses. That is, we observe that if we knew from which directions a point was seen from the given set of training images, then these directions can be used for not only better reconstruction, but also for different downstream applications such as uncertainty estimation and view selection.

In this work, we address this gap in the existing literature by modeling the \emph{the locations of likely observations} of a NeRF reconstruction of the scene and show its application in improving NVS quality and uncertainty estimation. We dub this the \textit{provenances} of a NeRF. As such, provenance is inherently linked to the triangulation quality of training cameras. However, determining the provenance of a point $\bm{x}$ is not easy as the locations that likely observe $\bm{x}$ depend on the training camera poses in a complex way. We illustrate this challenge using a camera pair (Figure~\ref{fig:tradeoff}). This is a well-known tradeoff in stereo matching~\cite{Okutomi_multiple_baseline_stereo, Praveen19, atanassovCamBaseline} and novel view synthesis~\cite{du2023cross, charatan23pixelsplat} literature: a small baseline leads to large stereo range error while a wider baseline can suffer from foreshortening and occlusion effects. As a result, the two settings should produce different sets of provenances. 

Despite the complexity accompanying provenance modeling, its definition gives rise to a probabilistic formulation of the provenances. If we have a probability distribution over observation locations for each $\bm{x}$, where a location $\bm{y}$ is assigned a high likelihood in the distribution if and only if it is likely to observe $\bm{x}$, we can treat provenances of $\bm{x}$ as the location samples with high likelihood from this distribution. Thus, if we model such a probability distribution for every point $\bm{x}$, we can obtain the provenances by sampling from the distributions. Inspired by recent works that use NeRFs to model additional 3D information~\cite{Zhi:etal:ICCV2021,kobayashi2022distilledfeaturefields, cen2023segment}, we model the provenance on top of NeRF representation using probabilistic methods~\cite{ho2020denoising, goodfellow2014generative,kingma2022autoencoding} with a learnable provenance distribution. Because the provenance distribution exists for every 3D point, this amounts to modeling a distribution of \emph{stochastic field} of provenances over $\R^3$. In our work, we extend implicit maximum likelihood estimation (IMLE)~\cite{li2018implicit} to model stochastic fields by adapting the objective to functional space. Furthermore, we derive an equivalent pointwise objective that can be efficiently optimized with gradient descent and use it to model the provenance field.
% to predict the provenance for all points in the scene. However, modeling the per-point provenance is not straightforward because we do not observe the full set of provenance during training. Motivated by the recent advance in probabilistic models~\cite{ho2020denoising, goodfellow2014generative,kingma2022autoencoding} that exhibit strong generalization capability, we reframe the modeling of provenance probabilistically as a 

% so that there is enough view overlap for feature matching and disparity calculation while ensuring that the stereo range error is not too high or it will likely result in inaccurate disparity estimation. \mika{Link your figure?} \george{because of this we model it as a distribution.}

% We claim that the per-point provenance of a NeRF can be used for different applications such as novel view synthesis and estimating the uncertainty of the captured process. 

% This motivates us to extract the \textbf{provenance} or the \emph{origin} of each point of NeRFs under sparse, unconstrained views.

% Given a pre-trained NeRF and its training camera poses, we define the set of provenances $\text{Prov}\paren{\bm{x}}$ for point $\bm{x}\in\R^3$ as a set of locations that are \textit{likely} to observe $\bm{x}$. As such, provenance is inherently linked to understanding the optimization of neural radiance fields, especially under a sparse setting. However, determining the provenance of a point $\bm{x}$ is not straightforward as the locations that likely observe $\bm{x}$ depend on the training camera poses in a complex way. This challenge is well-known in the literature of stereo matching~\cite{Okutomi_multiple_baseline_stereo, Praveen19, atanassovCamBaseline} and novel view synthesis~\cite{du2023cross, charatan23pixelsplat}. People often need to carefully select the baseline and orientations of the camera pairs so that there is enough view overlap for feature matching and disparity calculation while ensuring that the stereo range error is not too high or it will likely result in inaccurate disparity estimation. \mika{Link your figure?} \george{because of this we model it as a distribution.}

% \george{should I include this part?}
% While a natural group of candidates for provenance would be all the training cameras, as they are the places NeRF's optimization takes place, 3D consistency of NeRF also ensures that the provenances of $\bm{x}$ should generalize to unseen locations. This makes modeling NeRF's provenance challenging as there are no available ground truth provenances without enumerating all 3D positions and all possible locations that observe them. \mika{I'm a bit confused with this paragraph. What is the message you're trying to deliver?}

% Inspired by recent works that use NeRFs to distill additional 3D information from 2D supervision~\cite{Zhi:etal:ICCV2021,kobayashi2022distilledfeaturefields, cen2023segment}, we use NeRF to predict the provenance for all points in the scene. However, modeling the per-point provenance is not straightforward because we do not observe the full set of provenance during training. Motivated by the recent advance in probabilistic models~\cite{ho2020denoising, goodfellow2014generative,kingma2022autoencoding} that exhibit strong generalization capability, we reframe the modeling of provenance probabilistically as a \emph{stochastic process} which defines a \textit{probabilistic distribution} of provenance for each 3D point in the scene.

% Existing works however predict an additional \emph{scalar} field, that is, for each coordinate, there is a single deterministic output, e.g., semantics, features or normals, but in the case of directions, each point can be observed by multiple, very different directions and also varied number of cameras. Thus, instead of modeling a neural field that outputs a scalar value for each 3D point, we desire to model a stochastic process, where for each 3D point we output a \emph{distribution} of directions from where it was observed.

% To derive a stochastic process, a key challenge is modeling the distribution of directions for each 3D coordinate. One option is to use explicit probabilistic models with closed form densities such as Gaussians, where recent works have explored using this to model processes for point cloud reconstructions~\cite{} and single image~\mika{check this} depth estimation~\cite{}. Unfortunately, these distributions have limited expressivity, as they assume a single mode and have a fixed shape, which is not ideal for our case of modeling directions 3D points can be seen from a varied number and very different directions -- especially under the sparse, unconstrained view regime. Another option is to use implicit probabilistic models where the distribution is represented as a set of samples generated from a neural network. One choice of an implicit probabilistic model is GAN~\cite{}, but unfortunately, GANs can be prone to mode collapse and struggles in learning multimodal outputs~\cite{}, making them not ideal to model directions for our setting. To get around this conundrum, we propose to leverage IMLE~\cite{}, a implicit probabilistic model that is designed to handle multimodality, making it suitable to learn the distribution of directions for the sparse unconstrained setting.

% To model per-point provenance as a stochastic process, a key challenge is how to model the distribution of viewing source locations for each 3D coordinate. One option is to use explicit probabilistic models with closed-form densities, e.g. Gaussians~\cite{Sellan:Stochastic:2022}. Unfortunately, these distributions have limited expressivity as they have a fixed shape, and this is not ideal for modeling the distribution of per-point provenance as the distribution can be multimodal when a point is observed from multiple locations. Another option is to use implicit probabilistic models where the distribution is represented as a set of samples generated from a neural network. We extend implicit probabilistic models, specifically IMLE~\cite{li2018implicit} (implicit maximum likelihood estimation) to handle stochastic processes by adapting the original objective to functional space and show that it is equivalent to a pointwise matching of empirical and model samples. 

% One way to model the provenance process is to use explicit probabilistic models with closed-form densities, e.g. Gaussians~\cite{Sellan:Stochastic:2022}. Unfortunately, these distributions have limited expressivity as they have a fixed shape and are often unimodal. This renders them unsuitable for modeling the provenance process it can be multimodal when a point is observed from multiple locations. Instead, implicit probabilistic models represent the distribution as a set of samples generated from a neural network. Because of their implicit nature, they do not suffer from the abovementioned constraints. In our work, we extend implicit probabilistic models, specifically IMLE~\cite{li2018implicit} (implicit maximum likelihood estimation) to model stochastic processes by adapting the original objective to functional space and show that it is equivalent to a pointwise matching of empirical and model samples. 

We dub our method \methodname, a model that enriches any NeRF representation by additionally modeling the provenance field using a functional IMLE. We demonstrate that jointly optimizing the provenance distribution and the underlying NeRF can aid better novel view synthesis and scene understanding through its ability to estimate NeRF's uncertainty of the captured process.

% \mika{Not sure if we can have a stronger motivation here on directions -- triangulation.} \mika{Continuity figure: uncertainty/direction shouldn't change that much given epsilon change in the training images, i.e. sensor noise.}

% \mika{Bring up properties on why it is non-trivial. Each point is seen by a different number and multiple cameras. Hence unlike existing works, we cannot just model a field, ie a direct regression. Might need to bring up GT retrieval here, and have a property on why that isn't ideal. Hit on the properties that our method/technical contribution has -- ie here, we bring up the problems because of the properties.}

% \mika{Thus, we introduce XXX, where we model direction as a stochastic process. For each 3D point, it learns to predict a distribution of directions from where it was seen. Introduce technical novelties, generalization of cimle, etc.}

% \mika{We demonstrate that modeling a direction stochastic process enables multiple applications such as quantifying reconstruction uncertainty, view selection as well as improvement in novel view synthesis compared to state-of-the-art works. Not sure if here we want to say something about triangulation etc. This depends on the main pitch we want to hit later.}

% NeRF --> sparse views more practical (hit unconstrained cameras, ie wide baseline, in-the-wild setup) --> while recent works tackle this for better reconstruction, little have looked into uncertainty and best view selection (not sure how to best motivation application here).

% We realize that these can be derived from the training camera directions. That is, we ask ourselves, ``from where has each point been seen?", and this information comes for free given any pretrained nerf and training camera poses. We learn the directions

% Inspired by recent works that learn different semantic, feature, etc for different downstream applications, we also learn a direction field (process -- need to transition this). 

% Talk about method and technical contribution. why nontrivial.

% We show that this leads to uncertainty estimation from triangulation as in classical photogrametry, and best view selection...

% \begin{enumerate}
%     \item Growing popularity of NeRFs, touching different applications. 
%     \item For each 3D point in we want to learn an opacity and color given only supervision from posed 2D images.
%     \item A question that one can ask is ``from where has is the 3D points seen?" 
%     \item While commonly overlooked, this information comes for free just from the 2D poses and more importantly it can be used for multiple downstream applications.
%     \item In this work, we attempt to answer this question and learn to recover the training directions from where each coordinate is seen.
%     \item As each point is observed from multiple directions, different number of modes, then we need to model a distribution of directions for each 3D point.
%     \item Hence, we model direction as a stochastic process, where for each 3D point, it learns to predict a distribution of directions from where it was seen.
%     \item We show that modeling a direction stochastic process enables multiple applications such as quantifying reconstruction uncertainty and best view selection.
% \end{enumerate}

==> sections/viewpoint_optimization_old.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=\textwidth]{figures/view_select.jpg}
  \caption{\scriptsize{\textbf{(a)} PSNR and Area Size plots with the objective of maximizing the projected area of the target. \textbf{(b)} PSNR and Dot Product plots the objective of maximizing the dot product between the viewing angle and the target object's normal. The dotted lines denote the objective for the initial views. \textit{(Right)}  We show the final view comparison of our provenance-aided viewpoint selection compared to the baselines under the two objectives in scene 3. Notice that our method (in red) is able to arrive at an objective maximizing view while retaining reconstruction quality. On the other hand, both the retrieval and optimization baselines fail to balance between the two.}}
  \label{fig:area_normal_app}
\end{figure*}

\subsection{Criteria-based Viewpoint Optimization}
\label{sec_viewopt}
Finally, we show that our per-point provenance can be applied to criteria-based viewpoint selection, which leverages a neural rendering framework to determine the most favorable camera perspective based on a predefined criterion. For instance, this can encompass orienting the camera to align with the normal vector of a specified target or achieving a detailed close-up view of the target. The first criterion can be attained by minimizing the negative dot product between the camera's principal axis and the object's normal, whereas the second can be achieved through the minimization of the negative area of the 2D projection from a 3D plane encasing the object. A naive solution is to directly run gradient descent to optimize each corresponding objective loss \( \mathcal{L}_{\text{obj}} \).

We propose that the integration of two novel viewing loss functions within our model enhances the gradient's informativeness, thereby facilitating an approximation to the objective that is superior to conventional methods. More precisely, for each 3D point $\bm{x}_i$ lying on the object of interest, using our \methodname, we sample provenances $(t_1^{(i)}, \bm{d}_1^{(i)}), \dots, (t_K^{(i)}, \bm{d}_K^{(i)})$ from the distribution $\mathcal{D}_\theta(\bm{x}_i)$. Each distance-direction tuple sample $(t_j^{(i)}, \bm{d}_j^{(i)})$ gives a location $\bm{y}_j^{(i)} = \bm{x}_i - t_j^{(i)}\bm{d}_j^{(i)}$ from which $\bm{x}_i$ is seen, based on this, we define an additional loss $\mathcal{L}_{\text{select}} = -(\mathcal{L}_c + \mathcal{L}_d)$ as follows:
\begin{equation}
\small{
    \mathcal{L}_c  = \sum_i \max_j \| \bm{y}_j^{(i)} - \bm{c} \|_2^2; \; \mathcal{L}_d = \sum_i \max_j \left( R_{:,3}^\top \bm{d}_j^{(i)} \right),
}
\end{equation}
% \vspace{-0.2cm}
where \( [R|\bm{c}] \) denotes the camera pose, \( R_{:,3} \) corresponds to the third column of \( R \), reflecting the principal axis of the camera in the global coordinate system. Intuitively, \( \mathcal{L}_c \) seeks to align the camera center with the network's prediction, whereas \( \mathcal{L}_d \) aims to orient the principal axis of the camera toward the points. By running gradient descent on $\mathcal{L}_{\text{select}} + \mathcal{L}_{\text{obj}}$ from an initial viewpoint of the target object, our method can achieve better PSNR while moving closer to the desired criteria. We benchmark against two baselines: 1) a naive approach that exhaustively searches all training views to locate the one that minimizes \( L_{\text{obj}} \), and 2) a direct optimization approach that applies gradient descent solely on \( L_{\text{obj}} \) without considering \( L_{\text{select}} \).~\footnote{See supplementary for implementation details.}


% \begin{figure}[t]
%   \centering

%   \begin{subfigure}[b]{\linewidth}
%     \includegraphics[width=\linewidth]{figures/area_exp.png}
%     \label{fig:area_vis}
%   \end{subfigure}
  

%   \begin{subfigure}[b]{\linewidth}
%     \includegraphics[width=\linewidth]{figures/normal_exp.png}
%     \label{fig:normal_vis}
%   \end{subfigure}
  
%     \vspace{-0.4cm}
%   \caption{(a) Final view comparison of different methods, under the objective of making a close-look at the target object. (b) Final view comparison of different methods, under the objective of camera's principal axis aligned with the normal of the book. Direct optimization fails to capture the book in view, while ours achieve the orthogonal constraint with the book in view.}
%   \vspace{-0.4cm}
%   \label{fig:area_normal_vis}
% \end{figure}

\paragraph{Results.}
Both the quantitative (Left) and qualitative (Right) outcomes, presented in Figure~\ref{fig:area_normal_app}, demonstrate that our approach achieves a superior balance between PSNR and the intended objective~\footnote{To compute for PSNR at arbitrary poses, we train an oracle NeRF using the full captured sequence. We use Nerfacto~\cite{nerfstudio} as the oracle NeRF's representation.}. Although the naive retrieval baseline attains a higher PSNR, it fails to satisfactorily meet the desired objective, especially when training views are sparse and limited.


==> tables/ablation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lcc}
    \toprule
         & AP $\paren{\uparrow}$ & AUC $\paren{\uparrow}$ \\
         \midrule
         Deterministic Field & 0.163 &0.168 \\
        Gaussian-based w/ $C = 2$ & 0.537 & 0.539\\
        Gaussian-based w/ $C = 5$& 0.629 & 0.631\\
        VAE-based & 0.323 & 0.325\\\hline
        \methodname w/ Spatial Inv. $\mathcal{Z}$& \underline{0.742}	& \underline{0.744}\\
        \textbf{Ours} & \textbf{0.745} & \textbf{0.747} \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation Results on Scannet.}}
    \label{tab:ablation}
\end{table}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lcccc|cc}
%     \toprule
%          & $\substack{\text{Deterministic}\\\text{Field}}$ & $\substack{\text{Gaussian-based}\\\text{w/ }C = 2} $    & $\substack{\text{Gaussian-based}\\\text{w/ }C = 5} $ & VAE-based & $\substack{\text{\methodname}\\\text{w/ Spatial Inv.}}$  & \textbf{Ours}\\
%          \midrule
%          AP $\paren{\uparrow}$ & 0.163 & 0.537 & 0.629 & 0.323 & \underline{0.742} & \textbf{0.745}\\
%          AUC $\paren{\uparrow}$ & 0.168 & 0.539 & 0.631 & 0.325 & \underline{0.744} & \textbf{0.747}\\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Ablation Results on Scannet.}\vspace{-1cm}}
%     \label{tab:ablation}
% \end{table}

==> tables/nvs_tnt.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
    \toprule
         & PSNR $\paren{\uparrow}$ & SSIM $\paren{\uparrow}$ & LPIPS $\paren{\downarrow}$  \\
         \midrule
         % Vanilla NeRF~\cite{mildenhall2020nerf} & 17.19 & 0.559 & 0.457\\
        DDP~\cite{roessle2022depthpriorsnerf} & 19.18 & 0.651 & 0.361\\
         SCADE~\cite{scade}& 19.83&0.664&0.347 \\\hline
        Ours & \textbf{20.09}&\textbf{0.665}&\textbf{0.345}\\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Novel View Synthesis Results on Tanks and Temples Dataset.} SCADE numbers are obtained by running their released model weights. Scores for Vanilla NeRF and DDP are copied from SCADE.}
    \label{tab:reg_exp_tnt}
\end{table}

==> tables/unc_3dgs.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{l|cc}
    \toprule
         NLL$\paren{\downarrow}$& FisherRF & \textbf{Ours} \\
         \midrule
         \# 710 & 5.19 & \textbf{-3.93}\\
         \# 758 & 3.53 & \textbf{-6.04} \\
         \# 781 & 2.73 & \textbf{0.068}\\\hline
         Avg. & 3.82 & \textbf{-3.30}\\\bottomrule
    \end{tabular}
    \caption{\textbf{NLL Results for Triangulation Uncertainty.}\vspace{-0.7cm}}
    \label{tab:unc_3dgs}
\end{table*}

==> tables/unc_ause_experiment.tex <==
\begin{table*}[h]
    \centering
    \begin{tabular}{l|c|ccc||c|ccc}
         & \multicolumn{4}{c}{\textbf{Scannet}} & \multicolumn{4}{c}{\textbf{Matterport}} \\ 
         \cmidrule(lr){2-5}\cmidrule(lr){6-9}
         & Average & Scene 710 & Scene 758 & Scene 781 & Average & Room 0 & Room 1 & Room 2  \\
         CF-NeRF~\cite{CF-NeRF} & & & & & & & & \\
         Bayes' Rays~\cite{bayesrays}& 5.47& \underline{5.11} & 5.23 &6.07 & 5.49 & 5.67 & 5.77 & 5.91 \\\hline
        Ours & \textbf{-6.46} & \textbf{-1.98} & \textbf{-9.82} &\textbf{-7.58} & \textbf{-8.77} &\textbf{-12.5} & \textbf{-7.23} & \textbf{-6.58}\\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Negative Log-Likelihood Results} }
    \label{tab:my_label}
\end{table*}

==> tables/unc_retrieval.tex <==
\begin{table}
    \centering
    \begin{tabular}{lccc}
    \toprule
         NLL $\downarrow$ & Scene 710 & Scene 758 & Scene 781 \\ 
         \midrule
        Retrieval-based & 3.21 & 0.735 & -4.64\\
        Ours & \textbf{-0.283} & \textbf{-5.34} & \textbf{-7.58}\\
        \bottomrule
    \end{tabular}
    \caption{\footnotesize{\textbf{Uncertainty Estimation:} Negative log-likelihood on the Scannet dataset is reported.}}
    \label{tab:unc_nll_ret}
\end{table}

==> tables/unc_vanilla_nerf.tex <==
\begin{table}
    \centering
    \begin{tabular}{lccc}
    \toprule
          & Scene 710 & Scene 758 & Scene 781 \\ 
         \midrule
        Bayes' Rays &  \textbf{5.11}& 5.24 & 6.07\\
        Ours & 5.71 & \textbf{-2.53} & \textbf{2.16}\\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Uncertainty Estimation} The average negative log-likelihood on the Scannet Dataset. Both methods use vanilla NeRF as their backbones.}
    \label{tab:unc_nll_vanilla}
\end{table}
